Adjacent Pairs Exchange correction to the Random Phase Approximation

The Random Phase Approximation (RPA) is a widely employed post Hartree-Fock or DFT method, capable of capturing van der Waal interactions and other dynamic correlation effects at relatively low costs of $\mathcal O(N^3)$ in time and $\mathcal O(N^2)$ in memory, if calculated from imaginary time propagators. However, since it neglects anti-symmetrization RPA is biased, overestimating the correlation energy and bond lengths in general. The Second Order Screened Exchange offers amelioration by anti-symmetrizing one Coulomb interaction but it comes at considerable costs of $\mathcal O(N^5)$ in time and $\mathcal O(N^4)$ in memory, since it has to be calculated from the direct ring Coupled Cluster Doubles (drCCD) amplitudes. We propose a diagrammatic method, exchanging adjacent pairs in the RPA diagrams - hence its name - offering similar accuracy but with memory requirement of only $\mathcal O(N^2)$. The correction is calculated from imaginary time propagators similar to efficient RPA implementations. It can be calculated in $\mathcal O(N^5)$ steps in momentum space or $\mathcal O(N^4)$ steps in real space. It improves on SOSEX in the uniform electron gas for low densities, where correlation effects are stronger, and first calculations of lattice constants in solids are in excellent agreement with experiment.

==> ElectronicStructure.tex <==
%TODO: define orbitals

  \chapter{Electronic structure calculation}
    \section{Notation and units}
This work is mainly concerned with electronic properties. It is therefore
natural to choose units where the Schrödinger equation for electrons
appears as simple as possible. This is accomplished by atomic units
where the following constants are set to unity:
\begin{center}
\begin{tabular}{ll}
  electron mass & $m_e$ \\
  elementary charge & $e$ \\
  Coulomb's constant & $1/(4\pi\epsilon_0)$ \\
  reduced Planck's constant & $\hbar$ 
\end{tabular}
\end{center}
This renders the electron's Schrödinger equation for the hydrogen atom in a
particularly simple form:
\[
  \left(-\frac{\nabla^2}2 - \frac1r\right)\Psi = E \Psi
\]
Note, however, that the dimensions of the respective quantities must be
kept in mind although they do not appear explicitly. All energies are
given in Hartrees unless noted otherwise.

\begin{table}[h]
  \begin{center}
  \begin{tabular}{|l|l|}
    \hline
    \multicolumn{1}{|c|}{\textbf{Quantity}} &
    \multicolumn{1}{|c|}{\textbf{Symbol}} \\
    \hline
    scalars & $a,b,\ldots$ \\
    3-vectors & $\vec r, \vec r', \ldots$ \\
    spin and position combined $(\alpha,\vec r)$, where
      $\alpha \in \{\uparrow, \downarrow\}$&
      $\vec x, \vec x', \ldots$ \\
    matrices & $\vec A, \vec B, \ldots$ \\
    operators & $\hat A, \hat B, \ldots$ \\
    many-body wavefunction & $\Psi$ \\
    ground state Slater determinant & $\Phi$ \\
    spin oribital & $\psi_p$ \\
    index of general spin states (excited or unexcited) & $p,q,r,\ldots$ \\
    index of unexcited states & $i,j,k, \ldots$ \\
    index of excited states & $a,b,c,\ldots$ \\
    electron creation and annihilation operator for spin state $p$ &
      $\hat c^\dagger_p, \hat c_p$ \\
    hole creation and annihilation operator for spin state $i$ &
      $\hat i^\dagger, \hat i$ \\
    particle creation and annihilation operator for spin state $a$ &
      $\hat a^\dagger, \hat a$ \\
    creation and annihilation operator for a hole or a particle&
      $\hat p^\dagger, \hat p$ \\
    normal ordering operator & $N[\hat A\hat B\ldots]$ \\
    time ordering operator & $T[\hat A\hat B\ldots]$ \\
    imaginary unit $\sqrt{-1}$ & $\im$ \\
    \hline
  \end{tabular}
  \caption{Notation of physical quantities used herein}
  \label{tab:notation}
  \end{center}
\end{table}

  \section{The Schrödinger equation in condensed matter}
\begin{equation}
  \label{eqn:hamiltonian1st}
  \hat H = \underbrace{\sum_i \frac{-\nabla_i^2}2}_{\hat T} +
    \underbrace{\sum_{i,I}\frac{Z_I}{|\vec R_I - \vec r_i|}}_{\hat V_{\rm ne}} +
    \underbrace{
      \frac12\sum_{i\neq j} \frac1{|\vec r_i - \vec r_j|}
    }_{\hat V_{\rm ee}}
\end{equation}
  \section{The Hartree-Fock approximation}
difference of Hartree-Fock and the exact solution of the non-relativistic
time independent Schrödinger equation
\[
  E_{\rm C} = E_{\rm exact} - E_{\rm HF}
\]
Löwdin 1959

  \section{Density Functional Theory}



==> InterfacePinning.tex <==
  \chapter{Melting point calculations with Interface Pinning}
\section{\emph{Ab-initio} at finite temperature}
In single \emph{sb-initio} calculations using Hartree-Fock or
Density Functional Theory the positions of the atomic nuclei are assumed
to be fixed. Therefore, the resulting quantities, such as lattice constants
or atomization energies refer to zero temperature, even excluding
the zero point energy of the atomic vibrations. HF or DFT merely provides
a function $U(\vec R)$ to retrieve the energy of the system including its
electrons, given the positions of the atomic nuclei $\vec R$.
To calculate temperature dependent quantities, such as thermal expansion
coefficients or melting temperatures, we can treat the motion of the nuclei
classically to evaluate thermal expectation values of quantities of
interest $X(\vec R, \dot{\vec R})$:
\begin{equation}
  \langle X \rangle =
    \frac{
      \sum_{\vec R,\dot{\vec R}} X(\vec R,\dot{\vec R})\,
        e^{-\beta H(\vec R,\dot{\vec R})}
    }{
      \sum_{\vec R,\dot{\vec R}} e^{-\beta H(\vec R,\dot{\vec R})}
    }\,,
  \quad
  \textnormal{with }
    H(\vec R, \dot{\vec R}) = T(\dot{\vec R}) + U(\vec R)\,.
  \label{eqn:IP_ThermalAverage}
\end{equation}
$T(\dot{\vec R})$ is the classical kinetic energy of the
nuclei and $\beta = 1/\kB T$ is the inverse temperature in units of the
Boltzmann constant.
$H(\vec R,\dot{\vec R})$ is the classical Hamiltonian of the nuclei,
depending on its positions $\vec R$ and velocities $\dot{\vec R}$.
If the quantities of interest can be separated into a kinetic and
a potential part the sums can be separated as well. The kinetic part
can often be evaluated analytically since it is of a Gaussian form,
however, the integral over all configurations $\vec R$, given the potential
energy landscape $U(\vec R)$, is not trivial.

%TODO: Metropolis monte carlo reference
One way of evaluating this
integral is by means of a Metropolis Monte Carlo algorithm, which generates
(pseudo) random samples $\vec R_i$ of configurations that are asymptotically
distributed with a probability density function (PDF) proportional to
$e^{-\beta U(\vec R_i)}$. Thus, the thermal expectation value of a quantity
$X$ is approximately given by the average of the last values $X(\vec R_i)$.
The application of the Metropolis Monte Carlo algorithm to a potential
energy landscape $U(\vec R)$ calculated by an \emph{ab-initio} method is,
however, limited. The sampling algorithm places atoms at random positions,
which can impede the convergence of the self-consistent calculation
considerably.
It also takes a large number of iterations until the
sampling algorithm has covered a sufficiently large portion of the
configuration space for an accurate result. Finally, a considerable amount
of samples $\vec R$ is rejected from participating in the average, which can
only be done after the costly evaluation of $U(\vec R)$ from HF or DFT.

Another method to integrate the configuration space is by means of
a molecular dynamics simulation. Given the initial positions and velocities
of the atomic nuclei, the Hamiltonian equations of motions are solved
numerically, yielding a trajectory of configurations at discrete times
$\vec R(i\Delta t)$, where $\Delta t$ is the time step. The thermal average
of a quantity $X$ can then be approximated by the average over the last part
of the trajectory $X(\vec R(i\Delta t))$.
The ergodicity of the Hamiltonian dynamics
guarantees that the entire relevant phase space is eventually covered
by the trajectory of the system, regardless of the initial positions and
velocities of the nuclei.
In each iteration, $U(\vec R)$ and its gradient have to be evaluated from
a Hartree-Fock or DFT calculation. Unlike in the case of the Metropolis
algorithm, none of the calculated energies or forces have to be discarded.
Additionally, the quadratic equation of motion of the nuclei permits an
estimation of the HF or DFT wave function for the next iteration from the
previous two iterations, which considerably speeds up the convergence of the
self-consistent iterations in the respective \emph{ab-initio} calculation.
Finally, HF and DFT are both variational methods such that the gradient of
$U(\vec R)$ can be calculated analytically at hardly any extra costs employing
the \parencite{guttinger_verhalten_1932} theorem, also known as
Hellman-\-Feynman theorem.

Although the nuclei are heavy compared to electrons, a classical treatment
of their dynamics is not always justified, even at room temperature.
The frozen vibrational mode of N$_2$ and tunneling of protons are important
counterexamples. A path-integral molecular dynamics approach can be chosen in
these case, of course at considerably higher computational costs.
%TODO: find citation for path integral MD

    \section{Free energy}
There are cases where the relevant configuration space can by no
means be visited by the trajectory of a single molecular dynamics simulation on
the computer, not even a very long one. Crystallization or melting at a state
point of temperature and pressure close to the melting line are an example.
In such a first order phase transition there are two regions in configuration
%TODO: cite Landau-Ginzburg
space that are likely to be visited. In the example of melting, one region in
configuration space is where the atoms are in a crystalline configuration, the
other region is where the atoms are in a liquid configuration. One region, the
liquid, has a continuous rotational and translation symmetry on average, while
the other region has a discrete rotational and possibly\footnote{
A quasi-crystal does not exhibit translational symmetry.
} a discrete translational symmetry. Therefore, the two regions of
configuration space are not directly connected and a transition from one
region to the other region of configuration space can only occur collectively.
This makes a thermal transition very unlikely.
For instance, a simulation at the melting point, which starts from a
crystalline configuration will never melt and vice versa. Even in experiment,
a liquid can be supercooled to several degrees below freezing point, if it
is sufficiently free of impurities. It does not freeze due to the thermal
motion of its atoms until crystallization is induced externally, for
instance by shock.

The separation of regions in configuration space can be thought of as
deep basins in the potential energy landscape that are only connected by
saddle points high above the bottom of the respective basins. The
Boltzmann factor $e^{-\beta U}$ on the bottom of the basins is orders of
magnitude higher than that at the saddle points, which makes a spontaneous phase
transition very unlikely. If the system starts in a random configuration it
will evolve towards one of the deep basins in the potential energy landscape
and stay in the region of the respective basin\footnote{
  Eventually, it will pass the saddle points, exploring the entire configuration
  space. However, the half-life of staying in one region may be hundreds
  of orders of magnitude longer than the time evolving from
  a random configuration to an average configuration of one of the deep
  basin regions, usually referred to as \emph{equilibration} time.
  %FIXME: really 10^100? try and get some data
}.
Two such regions $A$ and $B$
are in \emph{coexistence}\index{coexistence}, if the probabilities of
evolving towards region $A$ and $B$ are the same:
\begin{equation}
  P(\vec R(T)\in A) = P(\vec R(T)\in B)\,,
  \label{eqn:IP_Coexistence}
\end{equation}
where the time $T$ is sufficiently large to explore the relevant
configuration space of either region $A$ or $B$.
An algorithm to determine whether a configuration is an element
of either region will be discussed in Section \ref{sec:IP_InterfacePinning}.
\begin{figure}
\begin{center}
\begin{asy}
  real beta = 5;
  real mu1 = 2, sigma2 = 1.5;
  real mu2 = 6, sigma1 = 0.5;
  real harmonic(real x, real mu, real sigma) {
    return exp(-beta*((x-mu)/sigma)^2/2)/sigma;
  }
  real pdf(real x) {
    return harmonic(x, mu1, sigma1) + harmonic(x, mu2, sigma2);
  }
  void drawAverageBox(
    real mu, real sigma, Label labelSigma="", Label labelU="", real sideU=+1,
    pen p = defaultpen
  ) {
    real U = (sqrt(pi)*(2^(3./2)*log(sigma)+sqrt(2)))/(2*beta^(3/2));
    real Sigma = (sqrt(2)*sqrt(pi)*exp((sqrt(2)*sqrt(pi)*log(sigma))/sqrt(beta)+sqrt(pi)/(sqrt(2)*sqrt(beta))))/sqrt(beta);
    path boundary = (mu-Sigma/2,0)--(mu-Sigma/2,exp(-beta*U))--
      (mu+Sigma/2,exp(-beta*U))--(mu+Sigma/2,0)--cycle;
    fill(boundary, lightgrey);
    label(labelSigma, (mu,0));
    label(labelU, (mu+sideU*Sigma/2,exp(-beta*U)));
    draw(boundary, p);
  }
  sizeRatio(240);
  drawAverageBox(
    mu1, sigma1,
    Label("$\Omega_A$", align=S),
    Label("$e^{-\beta\langle U\rangle_A}$",align=E), +1, blue
  );
  drawAverageBox(
    mu2, sigma2,
    Label("$\Omega_B$", align=S),
    Label("$e^{-\beta\langle U\rangle_B}$",align=E), +1, red
  );
//FIXME: increase number of plot points for better resolution of peak
  draw(graph(pdf, mu1-2*sigma1, mu2+2*sigma2));
  xaxis(Label("$\vec R$"));
  yaxis(Label("$e^{-\beta U(\vec R)}$"));
\end{asy}
\end{center}
\caption{
  A schematic plot of the configuration space for two phases $A$ and $B$
  at coexistence. It is equally likely to find the system in either phase,
  indicated by the area under each peak. The effective support $\Omega$
  is defined such that the area of the supported rectangle equals that
  under the respective peak.
}
\label{fig:IP_ConfigurationSpace}
\end{figure}
Figure \ref{fig:IP_ConfigurationSpace} sketches the configuration space
and the respective Boltzmann factors at coexistence. The integral
of the Boltzmann factors in a region corresponds to the
probability of finding the system in the respective region.
In order to relate the probability to quantities which can be measured,
we introduce the \emph{effective support}\index{effective support} $\Omega_A$
of a region $A$, defined such that the integral of the Boltzmann factors
in that region equals the product of the effective support and the
Boltzmann factor using the thermal average $\langle U\rangle_A$ of $U$
restricted to the region $A$.
In practice,
these are the thermal averages of the potential energy
when measured or calculated for a finite time
$T$, since a spontaneous transition to another region
is very unlikely to occur within that time.
We can then rewrite (\ref{eqn:IP_Coexistence}) to
\begin{equation}
  \Omega_A\,e^{-\beta \langle U \rangle_A} =
    \Omega_B\,e^{-\beta \langle U \rangle_B}\,.
  \label{eqn:IP_CoexP}
\end{equation}
%TODO: cite entropy discussion that Jeppe gave me
Finally, a probability is not a practical quantity to work with since it
is not extensive. Having a system consisting of two parts, the probability of
finding both for instance in the crystalline phase is the product of the
probabilities of finding each part in the crystalline phase, assuming
that the configurations of the two parts are sufficiently uncorrelated.
Taking the logarithm of (\ref{eqn:IP_CoexP}) gives an extensive quantity
and we get
\begin{equation}
  \langle U\rangle_A - TS_A =
    \langle U\rangle_B - TS_B\,,
  \label{eqn:IP_FreeEnergy}
\end{equation}
where $S_A=\kB\log\Omega_A$ is called \emph{entropy}\index{entropy} of
the system in a region $A$.
Above equation has the dimension of energy and the quantity
on either side is called
\emph{Helmholtz free energy}\index{Helmholtz free energy}. It is
the thermal analogous to energy since preferred regions have lowest
free energy as preferred configurations have lowest potential energy at
$T=0$\,K. Above equation still does not provide an algorithm of how to
compute the free energy difference between two phases. The previously
discussed means of evaluating thermal averages only allows us to evaluate
the thermal averages of the potential energies for each phase,
$\langle U\rangle_A$ and $\langle U\rangle_B$. For the solid/liquid
phase transition, Interface Pinning can be employed to evaluate the
difference of the Gibbs free energy per atom between the two phases
directly.
The \emph{Gibbs free energy}\index{Gibbs free energy} is the pendant of the
Helmholtz free energy at constant pressure, rather than constant volume.

\section{The Interface Pinning method}
\label{sec:IP_InterfacePinning}
Given an algorithm to classify configurations into crystalline and liquid
configurations,
coexistence could be calculated directly by setting up random configurations
and letting them evolve until they either form crystalline or liquid
configuration. If equally many random configurations evolve to either
phase, the phases are in equilibrium. This is, however, not a particularly
efficient algorithm since it requires thousands of steps for each
configuration and hundreds of initial configurations. It is also not
guaranteed that each initial configuration evolves to either to a liquid
or crystalline phase. It could be polycrystalline with various grain sizes,
which is not the result of a slow crystallization and therefore not desired.

%FIXME: show image of interface
Another direct way of calculation is to bring the two phases in contact,
having a mono-crystalline part, a liquid part and interfaces between the
phases, all in one simulation under periodic boundary conditions. This singles
out undesired polycrystalline phases and places the system on a saddle point
between the two phases of interest.
Starting at roughly half solid, half liquid, the system will either entirely
melt or solidify at constant temperature and pressure, depending on whether
the state point is above or below the melting line, respectively.
The average velocity of the interface will be zero at coexistence.
However, the simulation is not at equilibrium and a single calculation can
only be carried out until the system is entirely liquid or solid.
%TODO: cite: Zykova-Timan, Horbach and Binder, J. Chem. Phys. 133, 014705 (2010)

Interface Pinning improves on this method by imposing an additional bias
potential, coupled to an order parameter $Q(\vec R)$ which should be
proportional to the size of the crystalline phase:
\begin{equation}
   U'(\vec R) = U(\vec R) + \frac\kappa2 \left(Q(\vec R) - a\right)^2\,.
   \label{eqn:IP_BiasU}
\end{equation}
The strength of the bias potential is given by $\kappa$ and the desired
value of the order parameter is given by $a$, which is chosen close
to the order parameter of the initial half liquid, half solid configuration.
In a simulation above coexistence, the system will melt until the penalty
energy imposed by the bias potential is in balance with the free energy
gained from melting. If $\kappa$ is chosen strong enough, this balance
will occur before the system is entirely liquid and the system will stay
in this equilibrium for all practical considerations.
The situation is analogous in a
simulation below coexistence.
This converts the non-equilibrium situation of the two phase system into an
equilibrium situation, allowing to evaluate the thermal average
$\langle Q\rangle'$ of the order parameter $Q(\vec R)$ in the biased
dynamics, where the potential energy $U$ is replaced by the biased
potential energy $U'$. The average of the order parameter $Q$ will be
below the desired value $a$, if the system is simulated above the melting
line and the difference of $\langle Q\rangle'-a$ is related to the
difference of the Gibbs free energy per atom, called
\emph{chemical potential}\index{chemical potential}.

\subsection{Free energy of the two phase system}
We model the Gibbs free energy $G$ of the simulated system without the
bias potential as a function of
crystalline atoms assuming that the number of atoms in the planar interface
$N_{\rm i}$ as well as its free energy $G_{\rm i}$ is constant:
\begin{equation}
  G(N_{\rm c}) = N_{\rm c}\mu_{\rm c} + N_{\rm l}\mu_{\rm l} + G_{\rm i}\,.
  \label{eqn:IP_GibbsAtoms}
\end{equation}
$N_{\rm c}$ and $\mu_{\rm c}$ is the number of atoms and the chemical
potential in the crystalline phase and $N_{\rm l}$ and $\mu_{\rm l}$ is the
number of atoms and the chemical potential in the liquid
phase. $N=N_{\rm c}+N_{\rm l}+N_{\rm i}$ is the total number of atoms, which
is constant. The surface tension of the interface conserves the planar
interface as intially prepared. To justify the assumption of a constant
average number of atoms in the interface the crystal must be allowed
to grow and melt due to thermal fluctuations by at least one full layer
of atoms. Thus the strength of the bias potential $\kappa$ must be low
enough to allow that. Given an order parameter $Q(\vec R)$, which is
linear in the number of crystalline atoms, we can express the number
of crystalline particles by
\begin{equation}
  N_{\rm c} = \frac{Q(\vec R)}{\Delta q} + \textrm{const.}\,,
  \label{eqn:IP_CrystallineAtoms}
\end{equation}
where $\Delta q = \langle q\rangle_{\rm c} - \langle q\rangle_{\rm l}$ is
the difference of the average order parameter per atom between the liquid and
the crystalline phase.
Inserting (\ref{eqn:IP_CrystallineAtoms}) into (\ref{eqn:IP_GibbsAtoms})
yields the Gibbs free energy without the bias potential
as a function of the order parameter $Q$:
\begin{equation}
  G(Q) = \frac{\Delta\mu}{\Delta q} Q + \textrm{const.}
  \label{eqn:IP_GibbsQ}
\end{equation}

Above equation holds as long as the interface is planar and still present
in the system. Adding the bias potential changes the potential energy of
the system. However, it hardly changes the number of available configurations
of the system since the bias potential is relatively shallow compared
to the deep basins of either the fully crystalline or fully liquid regions.
Thus, the change of Gibbs free energy in the biased ensemble is equivalent to
the change of potential energy. From (\ref{eqn:IP_BiasU}) and
(\ref{eqn:IP_GibbsQ}), we get
\begin{equation}
  G'(Q) = \frac{\Delta\mu}{\Delta q} Q + \frac\kappa2(Q-a)^2\,.
  \label{eqn:IP_GibbsQBiased}
\end{equation}
Finally, we can retrieve the probability distribution of $Q$
from the free energy of the biased system as a function of $Q$
using the Gibbs free energy pendent of (\ref{eqn:IP_CoexP}) and
(\ref{eqn:IP_FreeEnergy}):
\begin{equation}
  \PDF(Q) \propto
    e^{-\beta G'(Q)} \propto
    e^{-\beta \kappa\left(Q-a+\Delta\mu/\kappa\Delta q\right)^2/2}\,.
\end{equation}
Thus, the order parameter $Q(\vec R)$ with the bias
potential enabled is Gaussian distributed and its expectation value and
its variance are
\begin{equation}
  \langle Q\rangle' = a - \frac{\Delta\mu}{\kappa\Delta q}\,,
  \qquad
  \langle Q^2 \rangle' - {\langle Q\rangle'}^2 = \frac{\kB T}\kappa\,.
\end{equation}
The former gives a direct relation between the thermal average of the order
parameter in the biased simulation and the Gibbs free energy difference
per atom $\Delta\mu = \mu_{\rm c} - \mu_{\rm l}$ between the liquid and the
crystalline phase. The latter is the statement of the equipartition theorem
that the average energy contained in the degree of freedom
offered by the bias potential, is $\kB T/2$.

\subsection{Order parameter for crystalinity}
Classifying whether a given configuration is an average configuration of
region $A$ or region $B$ is referred to as \emph{course graining}. For
crystallization we can for instance determine, whether the directions
to neighboring atoms are correlated.
%FIXME: Q6, and rho_k order paramter
%FIXME: dynamics on the order parameter, forces on rho_k possible in linear time

\section{Melting point of Na, Mg, Al and Si}
To keep the system at constant hydrostatic pressure and the crystal free of
strain the size of the simulation box may only change in the direction
perpendicular to the solid/liquid interface. %FIXME: cite Ulf's paper
We refer to this ensemble $Np_zT$ ensemble, assuming that the interface
is perpendicular to the $z$ axis.

\section{Interface mobility}
\subsection{Fluctuation dissipation theorem}
\subsection{Electrical analog}

\section{Summary and discussion}
* $N^3$ of ab-initio methods
* interface needs space, which worsens finite size effects
* MD at with more than one $k$ point difficult
* experimentally stable crystal phase may be unstable in DFT


==> Introduction.tex <==
  \chapter{Introduction}



==> LiquidMetalData.tex <==
\chapter[Data of the molten elements]{
  Data of the molten elements
}
\begin{sidewaystable*}[p]
\begin{tabular}{|r|l|r|l|r|rl|rl|r|r|c|r|l|r|l|r|rl|rl|r|r|}
  \cline{1-11}   \cline{13-23}
  \multicolumn{2}{|c|}{\multirow{2}{*}{Element}} &
    \multicolumn{1}{c|}{\multirow{2}{*}{$N$}} &
    \multicolumn{1}{c|}{\multirow{2}{*}{Electrons}} &
    \multicolumn{1}{|c|}{$\eps_{\rm max}$} &
    \multicolumn{1}{|c}{$T$} &
    \multicolumn{1}{c|}{[exp.]} &
    \multicolumn{1}{c}{$\rho$} &
    \multicolumn{1}{c|}{[exp.]} &
    \multicolumn{1}{c|}{$p$} &
    \multicolumn{1}{c|}{\multirow{2}{*}{$R$}} &
  \hspace*{2ex} &
  \multicolumn{2}{|c|}{\multirow{2}{*}{Element}} &
    \multicolumn{1}{c|}{\multirow{2}{*}{$N$}} &
    \multicolumn{1}{c|}{\multirow{2}{*}{Electrons}} &
    \multicolumn{1}{|c|}{$\eps_{\rm max}$} &
    \multicolumn{1}{|c}{$T$} &
    \multicolumn{1}{c|}{[exp.]} &
    \multicolumn{1}{c}{$\rho$} &
    \multicolumn{1}{c|}{[exp.]} &
    \multicolumn{1}{c|}{$p$} &
    \multicolumn{1}{c|}{\multirow{2}{*}{$R$}} \\
  \multicolumn{2}{|c|}{} &
     &
     &
    \multicolumn{1}{|c|}{[eV]} &
    \multicolumn{2}{|c|}{[K]} &
    \multicolumn{2}{c|}{[g/cm$^3$]} &
    \multicolumn{1}{c|}{[GPa]} &
     &
  \hspace*{2ex} &
  \multicolumn{2}{|c|}{} &
     &
     &
    \multicolumn{1}{|c|}{[eV]} &
    \multicolumn{2}{|c|}{[K]} &
    \multicolumn{2}{c|}{[g/cm$^3$]} &
    \multicolumn{1}{c|}{[GPa]} &
    \\
  \cline{1-11}   \cline{13-23}
 & & & & & & & & & & & & & & & & & & & & \\[-2ex]

3 & Li & 256 & 2s$^1$ & 140.0 & 470 & [454] & 0.534 & [0.512] & 0.29 & 0.69(0.04) & &  40 & Zr & 125 & 4s$^2$4p$^6$5s$^2$4d$^2$ & 229.9 & 2500 & [2128] & 6.305 & [5.8] & 0.01 & 0.80(0.03) \\
4 & Be & 125 & 2s$^2$ & 308.8 & 1850 & [1560] & 1.570 & [1.690] & -0.27 & 0.75(0.02) & &  41 & Nb & 125 & 4p$^6$5s$^1$4d$^4$ & 208.6 & 2900 &  & 7.669 &  & 0.96 & 0.87(0.02) \\
5 & B & 125 & 2s$^2$2p$^1$ & 318.6 & 2400 & [2349] & 2.245 & [2.08] & -1.69 & 0.08(0.06) & &  42 & Mo & 125 & 5s$^1$4d$^5$ & 224.6 & 3000 & [2896] & 9.330 & [9.33] & 0.42 & 0.86(0.02) \\
6 & C & 125 & 2s$^2$2p$^2$ & 273.9 & 5000 & [4800] & 1.374 & [1.37] & -1.59 & -0.08(0.04) & &  43 & Tc & 125 & 5s$^2$4d$^5$ & 228.7 & 2500 &  & 10.606 &  & -0.43 & 0.86(0.01) \\
 &  &  &  &  &  &  &  &  &  &  & &  44 & Ru & 125 & 5s$^1$4d$^7$ & 213.3 & 2800 & [2607] & 11.200 & [10.65] & 1.18 & 0.88(0.02) \\
11 & Na & 250 & 3s$^1$ & 62.1 & 370 & [371] & 0.941 & [0.927] & -0.02 & 0.84(0.01) & &  45 & Rh & 125 & 5s$^1$4d$^8$ & 229.0 & 2400 & [2237] & 10.807 & [10.7] & -1.86 & 0.86(0.04) \\
12 & Mg & 384 & 3s$^2$ & 98.5 & 900 & [923] & 1.581 & [1.584] & 0.07 & 0.91(0.02) & &  46 & Pd & 125 & 5s$^1$4d$^9$ & 250.9 & 1900 & [1828] & 10.380 & [10.38] & -1.32 & 0.92(0.02) \\
13 & Al & 256 & 3s$^2$3p$^1$ & 116.4 & 1000 & [933] & 2.352 & [2.375] & -0.27 & 0.85(0.03) & &  47 & Ag & 125 & 5s$^1$4d$^{10}$ & 249.8 & 1350 & [1235] & 9.320 & [9.320] & 0.98 & 0.88(0.02) \\
14 & Si & 125 & 3s$^2$3p$^2$ & 245.3 & 1700 & [1687] & 2.827 & [2.57] & 0.51 & 0.78(0.02) & &  48 & Cd & 125 & 5s$^2$4d$^{10}$ & 274.3 & 650 & [594] & 7.996 & [7.996] & 0.61 & 0.75(0.04) \\
15 & P & 125 & 3s$^2$3p$^3$ & 255.0 & 650 &  & 1.850 &  & -0.43 & -0.00(0.08) & &  49 & In & 125 & 5s$^2$5p$^1$ & 95.9 & 500 & [430] & 6.920 & [7.02] & -0.06 & 0.81(0.06) \\
16 & S & 125 & 3s$^2$3p$^4$ & 258.7 & 550 & [388] & 1.784 & [1.819] & 0.07 & 0.12(0.05) & &  50 & Sn & 125 & 5s$^2$5p$^2$ & 103.2 & 750 & [505] & 7.051 & [6.99] & 0.33 & 0.43(0.23) \\
 &  &  &  &  &  &  &  &  &  &  & &  51 & Sb & 125 & 5s$^2$5p$^3$ & 172.1 & 950 & [904] & 6.530 & [6.53] & 0.68 & 0.43(0.08) \\
19 & K & 125 & 3p$^6$4s$^1$ & 116.7 & 350 & [337] & 0.815 & [0.828] & 0.07 & 0.75(0.06) & &  52 & Te & 125 & 5s$^2$5p$^4$ & 175.0 & 750 & [723] & 5.700 & [5.70] & -0.64 & 0.15(0.15) \\
20 & Ca & 125 & 3p$^6$4s$^2$ & 266.6 & 1200 & [1115] & 1.378 & [1.378] & -0.44 & 0.80(0.03) & &  53 & I & 125 & 5s$^2$5p$^5$ & 175.6 & 500 &  & 3.250 &  & 0.16 & 0.03(0.12) \\
21 & Sc & 125 & 4s$^2$3d$^1$ & 154.8 & 1900 & [1814] & 2.800 & [2.80] & -0.38 & 0.50(0.11) & &   &  &  &  &  &  &  &  &  &  &  \\
22 & Ti & 125 & 4s$^2$3d$^2$ & 178.3 & 3900 & [1941] & 4.161 & [4.11] & -0.48 & 0.78(0.04) & &  55 & Cs & 125 & 5s$^2$5p$^6$6s$^1$ & 220.3 & 330 & [302] & 1.826 & [1.843] & 0.04 & 0.82(0.11) \\
23 & V & 125 & 3p$^6$4s$^2$d$^3$ & 263.7 & 2500 & [2183] & 5.773 & [5.5] & -0.13 & 0.78(0.03) & &  56 & Ba & 125 & 5s$^2$5p$^6$6s$^2$ & 187.2 & 1050 & [1000] & 3.338 & [3.338] & -0.41 & 0.55(0.09) \\
24 & Cr & 125 & 3p$^6$4s$^1$d$^5$ & 265.7 & 2600 & [2180] & 6.735 & [6.3] & -1.55 & 0.85(0.02) & &  57 & La & 125 & 5s$^2$5p$^6$6s$^2$5d$^1$ & 219.3 & 1280 & [1193] & 5.940 & [5.94] & -1.86 & 0.67(0.11) \\
25 & Mn & 125 & 4s$^2$3d$^5$ & 269.9 & 2400 & [1519] & 7.973 & [5.95] & 0.66 & 0.89(0.01) & &  72 & Hf & 125 & 5p$^6$6s$^2$5d$^2$ & 220.3 & 2600 & [2506] & 12.349 & [12] & -1.92 & 0.81(0.01) \\
26 & Fe & 125 & 3p$^6$4s$^2$3d$^6$ & 267.9 & 2400 & [1811] & 8.338 & [6.98] & 0.03 & 0.91(0.01) & &  73 & Ta & 125 & 5p$^6$6s$^2$5d$^3$ & 223.7 & 3450 & [3290] & 15.000 & [15] & 0.45 & 0.86(0.01) \\
27 & Co & 125 & 4s$^2$3d$^7$ & 268.0 & 1870 & [1768] & 8.924 & [7.75] & 0.22 & 0.91(0.00) & &  74 & W & 125 & 5p$^6$6s$^2$5d$^4$ & 223.1 & 3900 & [3695] & 16.803 & [17.6] & -0.78 & 0.85(0.04) \\
28 & Ni & 125 & 4s$^2$3d$^8$ & 269.5 & 2000 & [1728] & 8.189 & [7.81] & -0.17 & 0.90(0.01) & &  75 & Re & 125 & 6s$^2$5d$^5$ & 226.2 & 3650 & [3459] & 18.787 & [18.9] & 0.98 & 0.80(0.04) \\
29 & Cu & 125 & 4s$^1$3d$^{10}$ & 295.4 & 1480 & [1358] & 8.020 & [8.02] & -0.72 & 0.87(0.01) & &  76 & Os & 125 & 6s$^2$5d$^6$ & 228.0 & 3450 & [3306] & 19.741 & [20] & 0.46 & 0.86(0.03) \\
30 & Zn & 125 & 4s$^2$3d$^{10}$ & 276.7 & 760 & [693] & 6.570 & [6.57] & -0.61 & 0.56(0.06) & &  77 & Ir & 125 & 6s$^1$5d$^8$ & 210.9 & 2900 & [2719] & 19.275 & [19] & -0.91 & 0.71(0.03) \\
31 & Ga & 125 & 4s$^2$4p$^1$ & 134.7 & 420 & [303] & 6.082 & [6.095] & -0.67 & 0.80(0.03) & &  78 & Pt & 125 & 6s$^1$5d$^9$ & 230.3 & 2200 & [2041] & 18.532 & [19.77] & -1.00 & 0.88(0.03) \\
32 & Ge & 125 & 4s$^2$3d$^{10}$4p$^2$ & 310.3 & 1250 & [1211] & 5.600 & [5.60] & -1.46 & 0.78(0.07) & &  79 & Au & 125 & 6s$^1$5d$^{10}$ & 229.9 & 1470 & [1337] & 16.690 & [17.31] & 1.06 & 0.80(0.07) \\
33 & As & 125 & 4s$^2$4p$^3$ & 208.7 & 1300 & [1090] & 5.220 & [5.22] & 0.58 & -0.03(0.06) & &  80 & Hg & 125 & 6s$^2$5d$^{10}$ & 233.2 & 470 &  & 11.917 &  & 0.48 & 0.82(0.06) \\
34 & Se & 125 & 4s$^2$4p$^4$ & 211.6 & 550 & [494] & 3.838 & [3.99] & 0.16 & 0.02(0.11) & &  81 & Tl & 125 & 6s$^2$6p$^1$ & 90.1 & 600 & [577] & 11.220 & [11.22] & 0.53 & 0.91(0.05) \\
 &  &  &  &  &  &  &  &  &  &  & &  82 & Pb & 125 & 6s$^2$6p$^2$ & 98.0 & 900 & [601] & 10.671 & [10.66] & 0.48 & 0.84(0.05) \\
37 & Rb & 125 & 4p$^6$5s$^1$ & 121.9 & 340 & [312] & 1.460 & [1.46] & 0.01 & 0.74(0.10) & &  83 & Bi & 125 & 6s$^2$6p$^3$ & 105.0 & 580 & [545] & 10.050 & [10.05] & -0.27 & 0.33(0.01) \\
38 & Sr & 125 & 4s$^2$4p$^6$5s$^2$ & 229.4 & 1100 & [1050] & 2.375 & [2.375] & -0.24 & 0.81(0.07) & &  84 & Po & 125 & 6s$^2$6p$^4$ & 159.7 & 700 &  & 9.136 &  & -0.43 & 0.18(0.19) \\
39 & Y & 125 & 4s$^2$4p$^6$5s$^2$4d$^1$ & 202.6 & 1850 & [1799] & 4.359 & [4.24] & -0.47 & 0.56(0.04) & &  85 & At & 125 & 6s$^2$6p$^5$ & 161.4 & 600 &  & 6.500 &  & 0.31 & 0.05(0.10) \\
  \cline{1-11}   \cline{13-23}
\end{tabular}
  \caption{
    Correlation coefficients $R$ between the virial $W$ and potential energy $U$
    of the elements at the given state point $T,\rho$ close to the
    triple point. The values in parenthesis are the statistical uncertainties.
    $N$ is the number of atoms in the cubic or orthorhombic simulation box.
    The electronic configuration of the calculated electrons as well as the
    plane wave cutoff energies $\eps_{\rm max}$ are also listed. The experimental
    values were taken from
    \parencite{haynes2012crc}, \parencite{assael_reference_2012},
    \parencite{savvatimskiy_measurements_2005} and
    \parencite{haaland_graphite-liquid-vapor_1976}, where available.
  }
  \label{tab:details}
\end{sidewaystable*}




==> SimpleLiquids.tex <==

\chapter{Isomorphs in metal melts}
\section{Isomorph theory}
\section{The Direct Isomorph Check}
\section{High pressure behavior}
\section{Predicting the crystal structure from the liquid}
\subsection{The Inverse Power Law Ansatz}
\[
  U_{\rm IPL} =
    \sum_{i>j}\left(\frac{\sigma}{|\vec r_i-\vec r_j|}\right)^{3\gamma} +
    \textrm{const.}
\]
The variance of $U_{\rm IPL}$ is thus
\[
  \Var(U_{\rm IPL}) =
    \sigma^{6\gamma}\, \Var\left(\sum_{i>j}\frac1{|r_i-r_j|}\right)
\]
$\sigma$ fit such that
%TODO: update packing from Ulf's table
%TODO: metals separator in PTSE
%TODO: color scale in PTSE
%TODO: sigmas in reduced units in PTSE
%DONE: U_IPL/U_DFT correlation coefficient
%TODO: packing in table

\subsection{Comparison of physical properties}



==> Thesis-1.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalignT(-217.345120,208.437263)(-0.500000,0.249999){0.000000 1.000000 -1.000000 0.000000}{${\rm Im}(\omega)$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-15.982453,95.812649)(-0.500000,-0.750001){${\rm Re}(\omega)$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-107.141841,90.468103)(-0.500000,-0.796473){$|\vec k|>k_{\rm F}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-187.310019,107.781944)(-0.500000,0.203527){$|\vec k|<k_{\rm F}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-65.674852,157.584951)(0.000000,0.179999){$\mathcal C_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-250.871223,48.681914)(-1.000000,-0.820001){$\mathcal C_2$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-103.829466,18.956846)(0.000000,-0.500000){$\displaystyle G_0(\vec k,\omega)=\frac{\im}{\omega-\vec k^2/2+\im\eta_{\vec k}}$}


==> Thesis-10.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-10_0.pdf}%
}%
\special{pdf:q}%
\begin{picture}( 361.350000, 223.326582)%
\special{pdf:\ASYraw{
 -360.500000 -0.500000 m
 0.500000 -0.500000 l
 0.500000 222.992236 l
 -360.500000 222.992236 l
 -360.500000 -0.500000 l
h
 -308.152712 37.502371 m
 -237.263275 37.502371 l
 -237.263275 91.944762 l
 -308.152712 91.944762 l
 -308.152712 37.502371 l
h
W* n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalignT(-321.965855,29.125904)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{-8}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-321.965855,54.317552)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{-7}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-321.965855,79.509199)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{-6}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-321.965855,104.700847)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{-5}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-321.965855,129.892495)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{-4}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-321.965855,155.084143)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{-3}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-321.965855,180.275790)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{-2}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-321.965855,205.467438)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-348.994760,126.100774)(-0.500000,0.249999){0.000000 1.000000 -1.000000 0.000000}{$|$relative integration error$|$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-307.901185,24.985435)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$2$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-258.280177,24.985435)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-208.659169,24.985435)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$4$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-159.038162,24.985435)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$5$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-109.417154,24.985435)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$6$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-59.796147,24.985435)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$7$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-10.175139,24.985435)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$8$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-159.038162,11.138580)(-0.500000,-0.781250){1.000000 0.000000 0.000000 1.000000}{number of integration points}
\special{pdf:\ASYraw{
 -316.637994 29.017090 m
 -0.250000 29.017090 l
 -0.250000 222.242236 l
 -316.637994 222.242236 l
 -316.637994 29.017090 l
h
W n
}%
}%
\end{picture}%
\kern -361.350000pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{rgb}{1.000000,0.000000,0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-275.130598,80.557850)(0.000000,-0.500000){MP2d}
\definecolor{ASYcolor}{rgb}{0.000000,0.500000,0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-275.130598,70.143190)(0.000000,-0.500000){MP2x}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-275.130598,59.728530)(0.000000,-0.500000){RPA}
\definecolor{ASYcolor}{rgb}{0.000000,0.000000,1.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-275.130598,49.313870)(0.000000,-0.500000){APX}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-129.591509,143.724982)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{-5}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-129.591509,167.034306)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{-3}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-129.591509,190.343631)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-129.591509,213.652955)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-115.748368,139.584513)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$2$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-91.491688,139.584513)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-67.235008,139.584513)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$4$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-42.978328,139.584513)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$5$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-18.721648,139.584513)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$6$}
\special{pdf:q}%
\begin{picture}( 361.350000, 223.326582)%
\special{pdf:\ASYraw{
 -124.982356 143.188027 m
 -8.985281 143.188027 l
 -8.985281 212.854750 l
 -124.982356 212.854750 l
 -124.982356 143.188027 l
h
W n
}%
}%
\end{picture}%
\kern -361.350000pt%
\special{pdf:Q}%


==> Thesis-11.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-11_0.pdf}%
}%
\special{pdf:q}%
\begin{picture}( 361.509705, 223.326582)%
\special{pdf:\ASYraw{
 -360.659108 -0.500000 m
 0.500000 -0.500000 l
 0.500000 222.992236 l
 -360.659108 222.992236 l
 -360.659108 -0.500000 l
h
 -85.615459 37.300272 m
 -7.816931 37.300272 l
 -7.816931 69.960865 l
 -85.615459 69.960865 l
 -85.615459 37.300272 l
h
W* n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalignT(-318.267320,66.480016)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$0.004$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-318.267320,114.663287)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$0.005$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-318.267320,162.846557)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$0.006$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-318.267320,211.029827)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$0.007$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-347.926645,126.709104)(-0.500000,0.224793){0.000000 1.000000 -1.000000 0.000000}{fitted $E_{\rm c}^{\rm APX}$\,[eV]}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-290.913652,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$400$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-244.487253,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$500$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-198.060855,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$600$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-151.634456,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$700$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-105.208057,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$800$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-58.781659,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$900$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-12.355260,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$1000$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-157.437756,12.355240)(-0.500000,-0.750001){1.000000 0.000000 0.000000 1.000000}{largest $E_{\rm max}$ used for fit [eV]}
\special{pdf:\ASYraw{
 -312.953277 30.229204 m
 -0.745863 30.229204 l
 -0.745863 222.242236 l
 -312.953277 222.242236 l
 -312.953277 30.229204 l
h
W n
}%
}%
\end{picture}%
\kern -361.509705pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-51.758830,58.765263)(0.000000,-0.500000){0 terms}
\definecolor{ASYcolor}{rgb}{1.000000,0.000000,0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-51.758830,48.898103)(0.000000,-0.500000){1 term}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-109.471204,156.070858)(-1.000000,-0.500000){\vphantom{$10^4$}$0.003$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-109.471204,184.244108)(-1.000000,-0.500000){\vphantom{$10^4$}$0.005$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-109.471204,212.417359)(-1.000000,-0.500000){\vphantom{$10^4$}$0.007$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-139.130529,184.244108)(-0.500000,0.224793){0.000000 1.000000 -1.000000 0.000000}{$E_{\rm c}^{\rm APX}$\,[eV]}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-99.979752,151.930389)(-0.500000,-1.000000){\vphantom{$10^4$}$1^3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-78.575822,151.930389)(-0.500000,-1.000000){\vphantom{$10^4$}$2^3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-57.171891,151.930389)(-0.500000,-1.000000){\vphantom{$10^4$}$3^3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-35.767960,151.930389)(-0.500000,-1.000000){\vphantom{$10^4$}$4^3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-14.364030,151.930389)(-0.500000,-1.000000){\vphantom{$10^4$}$5^3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-57.171891,138.083534)(-0.500000,-0.781250){$k$-points}
\special{pdf:q}%
\begin{picture}( 361.509705, 223.326582)%
\special{pdf:\ASYraw{
 -104.937220 155.487778 m
 -8.979374 155.487778 l
 -8.979374 211.623769 l
 -104.937220 211.623769 l
 -104.937220 155.487778 l
h
W n
}%
}%
\end{picture}%
\kern -361.509705pt%
\special{pdf:Q}%


==> Thesis-2.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-2_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-42.854046,79.280959)(-0.500000,0.213937){$\vec q$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-73.058433,96.864052)(-0.500000,0.000000){$\vec k$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-74.419224,77.680341)(0.000000,-0.292667){$\theta$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-95.879939,67.417796)(-1.000000,-1.000000){$\Gamma$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-50.236926,26.459189)(0.000000,-0.817725){$k_{\rm F}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-6.651410,66.447624)(-0.500000,-0.822369){$k_z$}


==> Thesis-6.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-6_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-44.601025,77.152752)(-0.500000,0.213937){$\vec q$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-99.215657,95.393951)(-1.000000,-0.367061){$\vec k_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-99.215657,40.039888)(-1.000000,-0.367061){$\vec k_2$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-88.641685,70.059122)(0.000000,0.000000){$\Gamma$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-48.886974,25.620006)(0.000000,-0.817725){$k_{\rm F}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-6.651410,64.404544)(-0.500000,-0.822369){$k_z$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-309.344080,26.418269)(-1.000000,-0.367061){$\vec k_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-287.759668,99.842891)(-0.500000,0.258373){$u_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-256.336467,77.926573)(0.000000,-0.250001){$2\pi|\vec q|u_1$}


==> Thesis-9.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-9_0.pdf}%
}%
\special{pdf:q}%
\begin{picture}( 361.350000, 255.513035)%
\special{pdf:\ASYraw{
 -360.500000 -0.500000 m
 0.500000 -0.500000 l
 0.500000 255.058441 l
 -360.500000 255.058441 l
 -360.500000 -0.500000 l
h
 -85.119596 37.300272 m
 -7.321068 37.300272 l
 -7.321068 89.621458 l
 -85.119596 89.621458 l
 -85.119596 37.300272 l
h
W* n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalignT(-337.574315,78.539607)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$4$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-337.574315,142.802331)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$5$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-337.574315,207.065055)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$6$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-347.766940,142.802331)(-0.500000,0.224793){0.000000 1.000000 -1.000000 0.000000}{fitted $E_{\rm c}^{\rm APX}$\,[eV]}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-308.753631,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$400$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-259.393200,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$500$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-210.032769,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$600$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-160.672338,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$700$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-111.311907,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$800$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-61.951476,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$900$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-12.591045,26.202095)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$1000$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-166.842392,12.355240)(-0.500000,-0.750001){1.000000 0.000000 0.000000 1.000000}{largest $E_{\rm max}$ used for fit [eV]}
\special{pdf:\ASYraw{
 -332.188141 30.229204 m
 -0.250000 30.229204 l
 -0.250000 254.308441 l
 -332.188141 254.308441 l
 -332.188141 30.229204 l
h
W n
}%
}%
\end{picture}%
\kern -361.350000pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-51.261107,78.499583)(0.000000,-0.500000){0 terms}
\definecolor{ASYcolor}{rgb}{1.000000,0.000000,0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-51.261107,68.632423)(0.000000,-0.500000){1 term}
\definecolor{ASYcolor}{rgb}{0.000000,0.500000,0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-51.261107,58.765263)(0.000000,-0.500000){2 terms}
\definecolor{ASYcolor}{rgb}{0.000000,0.000000,1.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-51.261107,48.898103)(0.000000,-0.500000){3 terms}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-119.677670,202.948232)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$3.2$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-119.677670,232.925128)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$3.3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-138.386975,217.936680)(-0.500000,0.224793){0.000000 1.000000 -1.000000 0.000000}{$E_{\rm c}^{\rm APX}$\,[eV]}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-109.556560,183.819316)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$1^3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-85.633997,183.819316)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$2^3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-61.711434,183.819316)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$3^3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-37.788870,183.819316)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$4^3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-13.866307,183.819316)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$5^3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-61.711434,169.972461)(-0.500000,-0.781250){1.000000 0.000000 0.000000 1.000000}{$k$-points}
\special{pdf:q}%
\begin{picture}( 361.350000, 255.513035)%
\special{pdf:\ASYraw{
 -115.105555 187.257569 m
 -7.856205 187.257569 l
 -7.856205 246.987373 l
 -115.105555 246.987373 l
 -115.105555 187.257569 l
h
W n
}%
}%
\end{picture}%
\kern -361.350000pt%
\special{pdf:Q}%

